Roots in the semiring of finite deterministic dynamical systems

Finite discrete-time dynamical systems (FDDS) model phenomena that evolve deterministically in discrete time. It is possible to define sum and product operations on these systems (disjoint union and direct product, respectively) giving a commutative semiring. This algebraic structure led to several works employing polynomial equations to model hypotheses on phenomena modelled using FDDS. To solve these equations, algorithms for performing the division and computing $k$-th roots are needed. In this paper, we propose two polynomial algorithms for these tasks, under the condition that the result is a connected FDDS. This ultimately leads to an efficient solution to equations of the type $AX^k=B$ for connected $X$. These results are some of the important final steps for solving more general polynomial equations on FDDS.

==> tikzlibraryoodgraph.code.tex <==
%
% OODGraph: One Out-Degree Graphs library
%
% This library draws connected graphs with out-degree one. To draw unconnected OOD graphs, just draw separatedly their connected components
%
%\RequirePackage{etoolbox}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% This code below have been borrowed from etoolbox package  ----|          %
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%V% % % %
\newcommand*{\oodgraph@csxdef}[2]{\expandafter\xdef\csname#1\endcsname{#2}}
\newcommand*{\oodgraph@ifcsdef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}
\newcommand*{\oodgraph@ifcsundef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\expandafter
      \expandafter\@firstoftwo
    \else
      \expandafter\expandafter
      \expandafter\@secondoftwo
    \fi
  \else
    \expandafter\@firstoftwo
  \fi}
\newcommand*{\oodgraph@csuse}[1]{%
  \ifcsname#1\endcsname
    \csname#1\expandafter\endcsname
  \fi}
\newcommand{\oodgraph@cslet}[2]{%
    \expandafter\let\csname#1\endcsname#2}
\newcommand*{\oodgraph@csgundef}[1]{\global\oodgraph@cslet{#1}\relax}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % A %
% The above code have been borrowed from etoolbox package  ----| %
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%
% Version 0.1 (2019/05/25):
% - first public release
% Version 0.2 (2019/06/01):
% - added /.store in key
% - added /.default key
% - cleaned up code
% Version 0.3 (2019/06/14)
% - fixed drawing algorithm
% - points definitions are now saved in a list
% - the points list is emptied at the closing of the environment oodgraph
% Version 0.4 (2019/06/18)
% - now commands are completely scoped
% - redisigned the graph printing algorithm to take into account that now
%    everything is scoped
% Version 0.45 (2019/06/19)
% - added the option 'rotation angle'
% Version 0.46 (2019/06/20)
% - added the option 'node content'
% - added bridge to tikz and pgf when a key is not known
% - made the library independent of 'etoolbox' package (borrow
%    some code from the package)
% - added oodgraph@ prefix to all commands so to avoid conflicts with other
%    packages/libraries
% Version 0.47 (2019/06/28)
% - options 'oodgraph arrow' and 'oodgraph node' renamed into 'oodgraph edges' and 'oodgraph nodes' for more consistancy
% - fixed a bug with edges style
% - now '->' is the default edge style
% Version 0.48 (2019/07/14)
% - added a check in \addorigin to verifiy if the point has been defined before
% - some code polishing (eliminated the list oodgraph@more@options which is no
%    more used, deleted \oodgraph@resetkeys function and integrated its code
%    directly into the calling functions since its body contained only an \end{scope}
%    command, deleted several unuseful \expandafter commands)
% - explicited the definition of oodgraph@csxdef
% - partially rewritten the drawing routine for beards. Now it is much faster
% Version 0.50 (2019/07/15)
% - renamed style options 'oodgraph nodes' into 'nodes style' which is shorter and nicer
% - renamed style options 'oodgraph nodes' into 'nodes style' which is shorter and nicer
% - introduced the option 'loop style' which allows to style the loops
% - fixed a bug for the special case of cycles of order 2 which drawn the two edges
%   one over the other (obtening a double arrow). Thanks to François Doré for signalling
%   this.
% - bug fix: the beards to be wrongly oriented when the xshift key
%   was used in the addcycle command. Bug discovery and fix by François Doré
% - bug fix: when a cycle had only 2 nodes, they addresses where exchanged. Thanks
%   to François Doré for signalling this
% Version 0.51 (2024/02/02)
% - added the option 'rotation angle' for \addcycle
% - added the option 'attach margin' to make edges stop further away from the attach node to prevent them from intertwining when there are many of them
% - bug fix: when a cycle had only 1 node, the default angle of the beard does not match the shape of the loop
% - bug fix: the 'opening angle' option was wrongly computed
% - merged addbeard cases with 1 or 1+ nodes
% - changed the bend option in the case of a cycle of two nodes to preserve counterclockwise order for every case


\def\fileversion{0.51}
\def\filedate{2024/02/02}
\message{Library OODGraph}
\message{ v.\ \fileversion, \filedate}
% load tikz dependencies
\usetikzlibrary{calc, arrows.meta}
\makeatletter
\gdef\oodgraph@tmp{}
\gdef\oodgraph@points@list{}
%
% convenience routines to extract the prefix from a node path
%
\def\oodgraph@get@prefix@from@path@@#1-#2\pgf@eov{\xdef\oodgraph@tmp{\oodgraph@csuse{#1.origin}}}
\def\oodgraph@get@prefix@from@path#1{
\pgfutil@in@{-}{#1}
\ifpgfutil@in@% if there is a minus sign then it is a package defined point
\oodgraph@get@prefix@from@path@@#1\pgf@eov
\else% regular pgf/tikz point
\path(#1);\pgfgetlastxy{\XCoord}{\YCoord};
\xdef\oodgraph@tmp{(\XCoord,\YCoord)}
\fi
}
%
%  oodgraph@addtolist
%  #1 = name of the list to add to
%  #2 = object to be added
% Service function to append objects to lists
%
\newcommand*{\oodgraph@addtolist}[2]{%
   \expandafter\if\expandafter\relax\csname #1\endcsname\relax%
      \expandafter\expandafter\xdef\csname #1\endcsname{#2}%
   \else%
    \expandafter\xdef\csname #1\endcsname{\csname #1\endcsname,#2}%
\fi%
}
%
%  oodgraph@docslist@undeft
%  #1 = separator char
%  #2 = name of the list
% Service routine to \csundef all elements of the list
% 
\newcommand{\oodgraph@docslist@undef}[2][,]{%
%   #1 = separation char
%   #2 = list
   \def\dolist##1{\expandafter\@dolist##1#1\@eol}%
   \def\@dolist##1#1##2\@eol{%
   % process stuff here with ##1
   \oodgraph@csgundef{##1}
   \ifx\@eol##2\@eol\else\@dolist##2\@eol\fi}%
   \dolist{#2}%
}
%
\pgfkeys{/oodgraph/.search also={/tikz, /pgf}} %,/oodgraph/catch unknown}}%
%\pgfkeys{/oodgraph/.search also={/tikz,/pgf,/oodgraph/catch unknown}}%
\pgfkeys{%
/oodgraph/.cd,
%radius/.initial={1},
radius/.value required,
radius/.default={1},
radius/.store in=\oodgraph@radius,
radius,
%attach node/.initial={a->1},
attach node/.value required,
attach node/.default={a->1},
attach node/.store in=\oodgraph@attach@node,
attach node,
%nodes prefix/.initial={a},
nodes prefix/.value required,
nodes prefix/.default={a},
nodes prefix/.store in=\oodgraph@nodes@prefix,
nodes prefix,
%opening angle/.initial={120},
opening angle/.value required,
opening angle/.default={60},
opening angle/.store in=\oodgraph@opa,
opening angle,
rotation angle/.value required,
rotation angle/.default={0},
rotation angle/.store in=\oodgraph@rota,
rotation angle,
attach margin/.value required,
attach margin/.default={-1},
attach margin/.store in=\oodgraph@mgn@ratio,
attach margin,
nodes content/.value required,
nodes content/.default={$\bullet$},
nodes content/.store in=\oodgraph@node@content,
nodes content,
nodes@style/.style={ddsnode},
edges@style/.style={ddsedge},
loop@style/.style={looseness=8},
nodes style/.code=\pgfkeys{/oodgraph/nodes@style/.style={#1}},
edges style/.code=\pgfkeys{/oodgraph/edges@style/.style={#1}},
loop style/.code=\pgfkeys{/oodgraph/loop@style/.style={#1}},
semi thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={semi thick}},
thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={thick}},
ultra thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={ultra thick}},
edges color/.code=\pgfkeys{/oodgraph/edges@style/.append style={#1}},
nodes color/.code=\pgfkeys{/oodgraph/nodes@style/.append style={#1}},
}
%\pgfkeys{/oodgraph/.unknown/.code={%
%\ifx#1\pgfutil@empty\oodgraph@addtolist{oodgraph@more@options}{\pgfkeyscurrentname}\else\oodgraph@addtolist{oodgraph@more@options}{\pgfkeyscurrentname=#1}
%\fi}}
%
\newenvironment{oodgraph}[1][]{\begin{scope}[#1]}
{% closing the environment
% free all points definition in the current list
%\forcsvlist{\csgundef}{\oodgraph@points@list}
\expandafter\oodgraph@docslist@undef\expandafter{\oodgraph@points@list}
% free the points list
\gdef\oodgraph@points@list{}
% free temporary definitions
\gdef\oodgraph@tmp{}
\end{scope}}
%
\newcommand{\oodgraph@processkeys}[1][]{
\begin{scope}
\pgfkeys{/oodgraph/.cd,#1}
}
\long\def\oodgraph@drawcycle#1;{
\ifnum#1=1\oodgraph@drawcycle@\else%
{\ifnum#1=2\oodgraph@drawcycle@@{#1}\else%
\oodgraph@drawcycle@@@{#1}\fi}\fi%
% record circle center on points list and define it
\path(0,0);\pgfgetlastxy{\XCoord}{\YCoord};%
\oodgraph@ifcsundef{\oodgraph@nodes@prefix.origin}{%
% if undefined then add to the point list
\oodgraph@csxdef{\oodgraph@nodes@prefix.origin}{(\XCoord,\YCoord)}%
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix.origin}%
}%
{% if already defined then simply replace the old definition
\oodgraph@csxdef{\oodgraph@nodes@prefix.origin}{(\XCoord,\YCoord)}%
}%
\end{scope}
}
%
\newcommand{\oodgraph@drawcycle@}{
%\pgfcoordinate{myorigin}{\pgfpointorigin}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->1) at ({.01*cos(\oodgraph@rota)},{.01*sin(\oodgraph@rota)}){\oodgraph@node@content};
% save point on the list
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->1}
%\expandafter\oodgraph@csxdef\expandafter{\oodgraph@nodes@prefix->1}{(0pt,0pt)}
\oodgraph@csxdef{\oodgraph@nodes@prefix->1}{(0pt,0pt)}
% draw edge
\pgfmathsetmacro{\inloopvalue}{-130+\oodgraph@rota}
\pgfmathsetmacro{\outloopvalue}{130+\oodgraph@rota}
\draw[/oodgraph/edges@style]
(\oodgraph@nodes@prefix->1) edge[/oodgraph/loop@style,in=\inloopvalue,out=\outloopvalue] (\oodgraph@nodes@prefix->1);
}
\newcommand{\oodgraph@drawcycle@@}{
% second node
\pgfmathsetmacro{\oodgraph@half@radius}{.5*\oodgraph@radius}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->2) at ({-\oodgraph@half@radius*cos(\oodgraph@rota)},{-\oodgraph@half@radius*sin(\oodgraph@rota)}){\oodgraph@node@content};
% first node
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->1) at ({\oodgraph@half@radius*cos(\oodgraph@rota)},{\oodgraph@half@radius*sin(\oodgraph@rota)}){\oodgraph@node@content};
% register nodes
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->1}
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->2}
\oodgraph@csxdef{\oodgraph@nodes@prefix->1}{(-\oodgraph@half@radius,0pt)}
\oodgraph@csxdef{\oodgraph@nodes@prefix->2}{(\oodgraph@half@radius,0pt)}
% draw edges
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->1) edge[/oodgraph/edges@style, bend right] (\oodgraph@nodes@prefix->2);
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->2) edge[/oodgraph/edges@style, bend right] (\oodgraph@nodes@prefix->1);
}
\newcommand{\oodgraph@drawcycle@@@}[1]{
\pgfmathsetmacro\myangle{360.0/#1}
\foreach \i in {1,...,#1}{
  \pgfmathsetmacro\curangle{(\i-1)*\myangle+\oodgraph@rota}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->\i) at ({\oodgraph@radius*cos(\curangle)},{\oodgraph@radius*sin(\curangle)}){\oodgraph@node@content};
  \path(\oodgraph@nodes@prefix->\i); \pgfgetlastxy{\XCoord}{\YCoord};
  \oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->\i}
  \oodgraph@csxdef{\oodgraph@nodes@prefix->\i}{(\XCoord,\YCoord)}
}
%\wlog{list=\oodgraph@points@list}
\foreach \i in {1,...,#1}{
  \pgfmathsetmacro\mynext{ifthenelse(\i==#1,int(1),int(\i+1))}
  \draw[/oodgraph/edges@style] (\oodgraph@nodes@prefix->\i) -- (\oodgraph@nodes@prefix->\mynext);
}
}
\newcommand*{\addcycle}[1][]{%
\oodgraph@processkeys[#1]%
\oodgraph@drawcycle%
}
%
\def\addorigin#1;{%
\pgfutil@ifundefined{pgf@sh@ns@#1}{
\edef\mymsgtmp{No point named #1\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the point has been correctly defined via the standard TikZ interface.}
}{%
\path(#1);\pgfgetlastxy{\XCoord}{\YCoord};
\oodgraph@csxdef{#1}{(\XCoord,\YCoord)}%
\oodgraph@csxdef{#1.origin}{(\XCoord,\YCoord)}%
%\oodgraph@addtolist{oodgraph@points@list}{#1} % added v. 0.48
%\oodgraph@addtolist{oodgraph@points@list}{#1.origin} % added v. 0.48
}}
%
\newcommand{\addbeard}[1][]{%
\oodgraph@processkeys[#1]
\oodgraph@drawbeardlev
}
\def\oodgraph@drawbeardlev#1;{%
%\wlog{list=\oodgraph@points@list}
\oodgraph@drawbeardlev@@{#1}
\end{scope}}
\newcommand{\oodgraph@drawbeardlev@@}[1]{
% #1= number of nodes in the level
% check if the attachment node has been previously defined
\oodgraph@ifcsdef{\oodgraph@attach@node}{% then part
% if the attach node has been defined then
% find the root prefix and retrive the origin
\expandafter\oodgraph@get@prefix@from@path\expandafter{\oodgraph@attach@node}
\path[reset cm]\oodgraph@tmp;\pgfgetlastxy{\XOCoord}{\YOCoord};
\path[reset cm](\oodgraph@attach@node);\pgfgetlastxy{\XCoord}{\YCoord};
}% end of then part
{% if it is not defined, print an error message
\edef\mymsgtmp{No point named \oodgrap@attach@node\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the attachment node has been correctly defined or that there exists a addorigin command.}
}%
\begin{scope}[shift={(\XOCoord, \YOCoord)}]
% recompute coordinates of attach point in the new coordinate system
\pgfmathsetmacro\XCoord{\XCoord-\XOCoord}
\pgfmathsetmacro\YCoord{\YCoord-\YOCoord}
% compute angle wrt attachment point
\pgfmathsetmacro\myalphatmp{atan(\YCoord/(\XCoord+.01))}
\pgfmathsetmacro\myalpha{ifthenelse(\XCoord>=0,\myalphatmp,180+\myalphatmp)}
% compute lowest angle
\pgfmathsetmacro\mystartangle{\myalpha+\oodgraph@rota-(\oodgraph@opa/2)*ifthenelse(#1==1,0,1)}
% compute angle between two nodes
\pgfmathsetmacro\mystepangle{\oodgraph@opa/ifthenelse(#1==1,1,#1-1)}

\foreach \i in {#1,...,1}{
\pgfmathsetmacro\mycurangle{\mystartangle+(#1-\i)*\mystepangle}

\node[/oodgraph/nodes@style](\oodgraph@attach@node->\i) at ($(\oodgraph@attach@node)+({\oodgraph@radius*cos(\mycurangle)},{\oodgraph@radius*sin(\mycurangle)})$){\oodgraph@node@content};
\pgfmathsetmacro\mydrawcondition{ifthenelse(\oodgraph@mgn@ratio>=0,1,0)}
\ifnum\mydrawcondition=1%
{\draw[/oodgraph/edges@style] (\oodgraph@attach@node->\i) -- ($(\oodgraph@attach@node->\i)!\oodgraph@mgn@ratio!(\oodgraph@attach@node)$);}\else%
{\draw[/oodgraph/edges@style] (\oodgraph@attach@node->\i) -- (\oodgraph@attach@node);}\fi%

  % save points to points@list
  \path(\oodgraph@attach@node->\i); \pgfgetlastxy{\XCoord}{\YCoord};
 \oodgraph@addtolist{oodgraph@points@list}{\oodgraph@attach@node->\i}
 \oodgraph@csxdef{\oodgraph@attach@node->\i}{(\XCoord,\YCoord)}
}
\end{scope}
}
%
\makeatother
%
\endinput
